Revisiting Non-Specific Syndromic Surveillance

Infectious disease surveillance is of great importance for the prevention of major outbreaks. Syndromic surveillance aims at developing algorithms which can detect outbreaks as early as possible by monitoring data sources which allow to capture the occurrences of a certain disease. Recent research mainly focuses on the surveillance of specific, known diseases, putting the focus on the definition of the disease pattern under surveillance. Until now, only little effort has been devoted to what we call non-specific syndromic surveillance, i.e., the use of all available data for detecting any kind of outbreaks, including infectious diseases which are unknown beforehand. In this work, we revisit published approaches for non-specific syndromic surveillance and present a set of simple statistical modeling techniques which can serve as benchmarks for more elaborate machine learning approaches. Our experimental comparison on established synthetic data and real data in which we injected synthetic outbreaks shows that these benchmarks already achieve very competitive results and often outperform more elaborate algorithms.

==> sections/acknowledgments.tex <==

%\begin{ack}
%Use unnumbered first level headings for the acknowledgments. All acknowledgments go at the end of the paper before the list of references. Moreover, you are required to declare funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work). More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2020/PaperInformation/FundingDisclosure}. Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
%\end{ack}


\small{
\subsection*{Acknowledgments}
We thank our project partners the \emph{Health Protection Authority of Frankfurt}, the \emph{Hesse State Health Office and Centre for Health Protection}, the \emph{Hesse Ministry of Social Affairs and Integration}, the \emph{Robert Koch-Institut}, the \emph{Epias GmbH} and the \emph{Sana Klinikum Offenbach GmbH} who provided insight and expertise that greatly assisted the research. This work was funded by the Innovation Committee of the Federal Joint Committee (G-BA) [ESEG project, grant number 01VSF17034].
}

==> sections/review_response.tex <==
Regarding Lack of relevance for ML:
The main point of the paper is not the proposal of a new ML approach or beating the previous state-of-the-art, but that simple statistical techniques, which have been disregarded in previous works, are surprisingly hard to beat and, therefore, an important tool to assess any approach. We believe that this has a high relevance for ML researchers working in this area.
We are indeed working on ML approaches such as Sum-Product Networks for non-specific syndromic surveillance, and therefore, we surveyed the literature in both ML and statistics. 

Regarding Recent Related Work: We are happy to receive specific references to recent works in ML focusing on (in particular non-specific) syndromic surveillance.

(122 words)



%With respect to the concern of the lack of relevance for machine learning, we would like to point out that we are indeed working on machine learning approaches on non-specific syndromic surveillance, and in the course of this, we surveyed the available literature in both machine learning and statistics. To our surprise, there were almost no works that compared ML approaches to established statistical techniques, and, even more so, the statistical approches already seem to be hard to beat. We believe that this result has a high relevance for machine learning researchers working in this area (such as us).

%Regardless of this issue, the main point in this paper is not the proposal of a new ML approach or beating previous state-of-the-art,  but that the proposed statistical baselines are an important tool to assess any approach, as our comparisons show, and should not be disregarded in the future. For instance, we argue they are a prerequisite for checking the hypotheses of the reviewers that ML is not applicable for this task in general (R1), or that deep anomaly detection methods should work relevantly better (R3). Of course, such investigations would be the next steps, but these investigations would probably deserve a separate paper. In this paper, we included comparisons to the existing state-of-the-art known to us in *non-specific* syndromic surveillance on accepted benchmark datasets for this task in order to allow for reproducibility and comparability. Our non-verifiable, preliminary experiments on non-publishable real data confirm the results, but would in our opinion only distract from the focus of the paper.


%With respect to the criticism that newer works are lacking: we are happy on receiving specific references to works on all aspects of syndromic surveillance. In particular, we would be interested in all recent references that are relevant to our focus on non-specific syndromic surveillance, for which we are currently not aware of more recent works in Machine Learning.



==> sections/table_results.tex <==
\begin{table*}[!htb]
    \centering
    %\footnotesize
    \caption{Results on the synthetic data.}
    
\resizebox{\linewidth}{!}{%
\begin{tabular}{lr | lr}
\toprule
algorithm & $AAUC_{5\%}$ &  algorithm & $AAUC_{5\%}$\\
  \midrule
        WSARE 2.0 (min. $p$-value)&                        3.054   & DMSS ($sup=3$, $w=30$) &              3.270 \\
        WSARE 2.5 (min. $p$-value)&                          1.359 & DMSS ($sup=3$, $w=90$)   &             3.078 \\
        WSARE 3.0 (min. $p$-value)&                          0.925  & DMSS ($sup=3$, $w=180$)   &             3.384 \\
  \midrule
        WSARE 2.0 (permutation test)&                          3.922  & DMSS ($sup=5$, $w=30$) &                 2.935 \\
        WSARE 2.5 (permutation test)&                          1.656  & DMSS ($sup=5$, $w=90$)   &              2.838\\
        WSARE 3.0 (permutation test)&                          1.348  & DMSS ($sup=5$, $w=180$)   &              3.057\\
  \midrule
        WSARE 2.0  (imported $p$-values) &                          4.943  & DMSS ($sup=7$, $w=30$)    &             2.839\\
        WSARE 2.5  (imported $p$-values) &                          1.966  & DMSS ($sup=7$, $w=90$)      &           2.702\\
        WSARE 3.0  (imported $p$-values)&                          1.608  & DMSS ($sup=7$, $w=180$)      &           2.955\\
          \midrule%\midrule
    Gaussian  &                          0.971  & Eigenevent (rerun)&                          5.721 \\
    Poisson  &                         1.329  & Eigenevent (imported $p$-values) &                          4.596 \\
    Negative Binomial  &                          1.031   \\
    Fisher's test  &                                        1.057  &   \\
\bottomrule
\end{tabular}
}
\label{tab:results_synthetic_approaches}
\end{table*}

==> sections/table_results2.tex <==



\begin{table}[t!]
    \centering
    %\footnotesize
    \caption{Results on the synthetic data.}
%\resizebox{\linewidth}{!}{%
\begin{tabular}{lr}
\toprule

algorithm & $AAUC_{5\%}$\\
  %\midrule
    %Control Chart &                          5.090 \\
    %Moving Average &                          6.977  \\
    %Linear Regression &                          3.596  \\
  \midrule
        WSARE 2.0 (min. $p$-value)&                        2.963  \\
        WSARE 2.5 (min. $p$-value)&                          1.321 \\
        WSARE 3.0 (min. $p$-value)&                          0.898  \\
  \midrule
        WSARE 2.0 (permutation test)&                          3.805   \\
        WSARE 2.5 (permutation test)&                          1.614  \\
        WSARE 3.0 (permutation test)&                          1.325 \\
  \midrule
        WSARE 2.0  (imported $p$-values) &                          4.925 \\
        WSARE 2.5  (imported $p$-values) &                          1.931 \\
        WSARE 3.0  (imported $p$-values)&                          1.610  \\
  \midrule
        DMSS ($sup=3$, $w=30$) &              3.310   \\
        DMSS ($sup=3$,$w=90$)   &             3.011 \\
        DMSS ($sup=3$,$w=180$)   &             3.433 \\
  \midrule
        DMSS ($sup=5$, $w=30$) &                 2.985   \\
        DMSS ($sup=5$,$w=90$)   &              2.817 \\
        DMSS ($sup=5$,$w=180$)   &              3.070  \\
  \midrule
        DMSS ($sup=7$, $w=30$)    &             2.819 \\
        DMSS ($sup=7$,$w=90$)      &           2.764 \\
        DMSS ($sup=7$,$w=180$)      &           2.996  \\
  \midrule
    Eigenevent (rerun)&                          4.993  \\
    Eigenevent (imported $p$-values) &                          4.391 \\
   \midrule
      Gaussian &                          0.941  \\
      Poisson  &                         1.347  \\
      Negative Binomial &                          0.966 \\
      Fisher's test &                                        1.057 \\
\bottomrule
\end{tabular}
%}
\label{tab:results_synthetic_approaches}
\end{table}

